Experience-Based Heuristic Search: Robust Motion Planning with Deep Q-Learning

Interaction-aware planning for autonomous driving requires an exploration of a combinatorial solution space when using conventional search- or optimization-based motion planners. With Deep Reinforcement Learning, optimal driving strategies for such problems can be derived also for higher-dimensional problems. However, these methods guarantee optimality of the resulting policy only in a statistical sense, which impedes their usage in safety critical systems, such as autonomous vehicles. Thus, we propose the Experience-Based-Heuristic-Search algorithm, which overcomes the statistical failure rate of a Deep-reinforcement-learning-based planner and still benefits computationally from the pre-learned optimal policy. Specifically, we show how experiences in the form of a Deep Q-Network can be integrated as heuristic into a heuristic search algorithm. We benchmark our algorithm in the field of path planning in semi-structured valet parking scenarios. There, we analyze the accuracy of such estimates and demonstrate the computational advantages and robustness of our method. Our method may encourage further investigation of the applicability of reinforcement-learning-based planning in the field of self-driving vehicles.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> rest.tex <==
\section{Introduction}

Robust autonomous systems should cope well with the uncertainty inherent to interactions with their surrounding environment. During sensing, uncertainties are introduced via sensor limitations, noise or imperfect self-localization. During acting, the visited states of an environment cannot be predicted deterministically from the actuation input since the definition of such a prediction model would require a fully observable environment.


\begin{figure}[t!]
	
	\centering
	\captionsetup[subfigure]{width=0.44\columnwidth}
	\subfloat[Unstructured environment: non-holonomic constraints and obstacle avoidance]
		{	\includegraphics[width=0.48\columnwidth]{pictures/sample_15.pdf}  }
	\subfloat[Structured environments: goal region (hatched rectangle) and non-holonomic constraints.  ] 
		{	\includegraphics[width=0.48\columnwidth]{pictures/rendersample_73.pdf} }

	\caption{Preliminary path planning results for two different scenarios generated with a Deep Q-Network using a greedy policy. The neural network policy was trained with Double Deep Q-Learning in a continuous state and discrete action space. Positive rewards were given for reaching the goal, negative rewards for collisions and direction changes. The learned Q-functions may be used as a unified heuristic function in existing path planning algorithms.} \label{fig:heuristic_learning}.	
\end{figure}


It is widely accepted that human cognition, in contrast to using a deterministic model, relies on probabilistic concepts such as Bayesian inference to orientate itself in an uncertain world. A variety of approaches exist which apply such principles in the development of perception and motion planning approaches for autonomous vehicles. Kalman and particle filtering allow to continuously integrate sensor measurements and actions into a probabilistic belief state of a system. With partially observable Markov decision processes (POMDP) one can model environmental interactions based on probabilistic state transition and observation functions in combination with a reward definition describing the benefit of performing a certain action in a specific state.

However, to be capable of handling the extensive computational cost inherent to belief space calculations, existing probabilistic motion planning approaches for autonomous vehicles consider only a subset of uncertainty types, use simpler probabilistic models and are mostly designed for one specific scenario such as highway maneuvering or intersection crossing. Consequently, they are limited in terms of applicability in today's autonomous driving architectures. Especially, urban scenarios such as crossing a crowded intersection and driving in residential areas with many children are characterized by a high uncertainty regarding the intention of traffic participants and sensing inaccuracies due to a potentially occluded field of view. The motion planning architecture of an autonomous vehicle should take into account all of these aspects of uncertainty to avoid executing a potentially risky maneuver.

Humans address the uncertainty in environmental interaction by learning the optimal action for a current belief in a continuous cycle of observation, action and reward steps. They anticipate the effects of their actions and base future decisions on learned experiences. Based on this principle in reinforcement learning an agent learns optimal policies in an agent-environment interaction. Existing reinforcement learning approaches for autonomous driving mostly focus on the behavior level to solve only a single simpler driving scenario such as a lane change, or they apply end-to-end learning hampering the integration into today's autonomous driving architectures.

In contrast, we want to apply Deep Reinforcement Learning in more complex scenarios exhibiting high environmental uncertainty  by benefiting from recent advances in the field of belief space planning with neural-networks. By using function approximators such as Deep Neural Networks for reinforcement learning, no exact POMDP model is required. State transition and observation rules are deduced during the agent's environmental interaction, which in principle allows to learn policies for high dimensional and continuous state spaces. Having no restrictions regarding the dimension of the underlying belief space these approaches are promising for application in the field of probabilistic motion planning, especially for autonomous driving, where a generalization of a probabilistic motion planner to the multitude of possible traffic scenarios is required. 





\section{Topic}
In this thesis we approach probabilistic planning for autonomous driving using Deep Reinforcement Learning for POMDP problems. State of the art approaches for probabilistic motion planning are limited in terms of applicability to different scenarios. To be capable of handling the extensive computational cost inherent to belief space calculations, they consider only a subset of uncertainty types, apply simpler probabilistic models and are mostly designed for one specific scenario such as highway maneuvering or intersection crossing using a discrete action set and low-dimensional state space. Furthermore, they do not allow for a flexible integration of an arbitrary uncertainty model, such as a learned model describing the uncertainty in pedestrians' intentions, while at the same time considering measurement and actuation uncertainty.   

In contrast, approaching belief space planning with Deep Reinforcement Learning brings the following benefits
\begin{itemize}

	\item \textbf{High-dimensional model-free belief space planning:} No exact definition of a POMDP model of the whole traffic scenario with transition and observation functions is required. Given an arbitrary environmental definition including e.g. perception inaccuracies or uncertainties in intention estimation, the corresponding POMDP model is deduced during training. This enables a better generalization to different driving scenarios and allows for a flexible integration of complex, even learned, probabilistic models.
	\item \textbf{Heuristic Learning:} We can learn probabilistic heuristic functions represented by a state-action-value function which can be integrated into existing kinematic path planning concepts, beneficial for instance in narrow parking scenarios. Preliminary results of investigating the planning capability of a Deep Q-Network are given in figure \ref{fig:heuristic_learning}.
	\item \textbf{Trajectory generation:} By using a setting with continuous kinodynamic actions, we can extend	the	approach towards a 	versatile uncertainty planner at trajectory	level.
	\item \textbf{Experience based planning:} After training, planning is based on experience. Specifically, the agent selects the action which performs best with respect to the learned expectation of the future environmental development.  This limits the computational cost for a planning step in belief space to the time needed for forward evaluation of the neural network. 
	\item \textbf{Improving interaction-aware planning:} An interaction-aware planner considers the reactions of other traffic participants within the planning process. To address the problem that drivers mutually influence each other, commonly certain restrictive assumptions, such as setting a constant velocity for a certain time period, must be made.
	In contrast, when using reinforcement learning, only the intention models of the traffic participants are needed for the simulation. Without any further restrictions, we expect the agent to adapt an interaction-aware strategy during environmental interaction in the training process.
\end{itemize} 

 
The previously mentioned benefits are especially relevant in challenging urban scenarios. For instance, parallel parking in narrow gaps as this is commonly impeded by high sensing uncertainty due to the partially occluded field of view of the sensors as well as possible inaccuracies regarding actuation. Furthermore, we expect to better handle  scenarios in which a high uncertainty regarding estimated intentions of pedestrians and other vehicles is given such as crossing of crowded intersections or driving in residential areas with playing children.

\section{Challenges}
Finding a neural network architecture which is able to learn a suitable internal belief state representation will be a key challenge of this thesis. In addition, the architecture must be capable of performing a planning process within the network. Initial ideas to address these problems are given in sections \ref{sec:planning} and \ref{sec:POMDP}.

To allow our approach to generalize well to different driving scenarios, we will have to appropriately design the network input which may consist of the environmental observation, the action history as well as fixed parametric constraints such as the maximum allowed acceleration or number of moves. Additionally, the design must support learning of a task-relevant feature representation based on environmental observations. We present approaches for these challenges in sections \ref{sec:feat_rep} and \ref{sec:net_arch}.

Furthermore, we require a training procedure which ensures a complete exploration of the observation and belief space by the reinforcement learning agent. This requires a simulation environment which provides the large amount of training data without significant limitations regarding processing time and costs. Sections \ref{sec:training} and \ref{sec:sim_env} discuss different ways of meeting these requirements.


\section{Related Work}
We discuss the state of the art methods most relevant to the topic and summarize their main drawbacks.

\subsection{Path Planning}
Path planning approaches for autonomous vehicles in unstructured environments are divided into state lattice and sampling based incremental search methods \cite{katrakazas_real-time_2015-1}. 

\subsubsection{Lattice Planning}

State lattice planning methods are based on a discretization of the configuration space of the vehicle. The Hybrid A* algorithm \cite{dolgov_path_2010} extends the conventional A* algorithm towards a continuous state representation in each grid cell. This allows for generation of kinematically feasible paths. However, as only a discretized number of steering actions is applied at each expansion the resulting path is likely to exhibit a discontinuous curvature. Therefore, Hybrid A* planners require in general a subsequent optimization step to obtain a drivable path \cite{dolgov_practical_2008}.

A heuristic function guides the state exploration. This metric also referred to as cost-to-go is commonly given by the maximum of a non-holonomic heuristic without obstacles and a holonomic heuristic with obstacles \cite{du_path_2016, dolgov_path_2010}. However, dealing with both structured and unstructured environments with lattice based planners is impeded due to the discretized nature of the state space. \citet{fassbender_motion_2016} propose a heuristic which guides the expansions towards a road graph with the drawback of needing additional parameter fine-tuning.


\subsubsection{Sampling Based}

Sampling based methods like RRT explore the reachable configuration space by growing a tree rooted at the initial configuration \cite{lavalle_planning_1999}. A random vertex is iteratively selected and a steering function returns the control commands to connect the vertex with its parent with a dynamically feasible path. Under certain assumptions it can be shown that the RRT algorithm is probabilistically complete. Exploratory behaviour based on a heuristic functions yields faster expansion towards the goal but cannot ensure probabilistic completeness. \citet{karaman_sampling-based_2011} demonstrate that with the RRT* algorithm a suboptimal solution is obtained with probability one by steadily rewiring the graph to retain only minimum cost paths.   

Drawbacks of RRT* for autonomous driving are the resulting jerky paths, and the dependency of the convergence rate on the expansion metric as with lattice based methods. 


%\rework{
%\cite{kiss_effective_2017-2}
%do we need this?
%}
\subsection{Probabilistic Motion Planning}

Probabilistic motion planning approaches may be divided into general approaches from the field of robotics and methods specifically designed for autonomous driving. 

\subsubsection{General}
\citet{christensen_motion_2017} propose a belief space planning method to find a locally optimal solution to the POMDP problem in continuous domains. An initial solution is given by an RRT planner. Then, differential dynamic programming leads to a locally optimal solution. The method does not handle uncertainty in sensing and computation time is intractable for real-time usage.

In a different class of probabilistic planning algorithms the computations in belief space are approximated via sampling. \citet{chiang_runtime_2016} present an online motion planning method dealing with a large number of stochastically interacting obstacles, despite the presence of uncertainty in obstacle localization. They use an RRT algorithm in state-time space to find a path through MC sampled obstacle trajectories. However, they do not consider uncertainty in robot dynamics.


\subsubsection{Autonomous Vehicles}
\citet{bry_rapidly-exploring_2011} propose a probabilistic motion planning method based on the RRT* algorithm. They mention that the uncertainty prediction via Kalman filter is only reasonable during online path execution when valid measurements are acquired. Thus, the authors derive a \textsl{closed loop distribution over planned trajectories} by incorporating the tracking error of the stabilizing controller. Additionally, they use the RRT* algorithm extended by a belief space representation for planning. Using Dubin's vehicle dynamics and a LIDAR sensor model, they plan in a simple unstructured environment. However, their method uses linearised systems with Gaussian noise properties and cannot account for uncertainty in obstacle positions.
	  

\citet{lenz_heuristic_2015} extend their method and incorporate \textsl{uncertainty in obstacle perception and actuation} into a heuristic search by adding a success probability computed in belief space to the heuristic function of a A* planner. However, the integration over the continuous belief space must be approximated with sampling and is computationally intensive. Furthermore, their algorithm does not allow for a straightforward integration of dynamic objects or predicted intentions.

%\rework{
% \cite{ Yang et al 2016}
%add 
%}

In \cite{bai_intention-aware_2015}, they account for uncertainty in \textsl{pedestrians' intentions } by modelling the interaction between pedestrians and an autonomous vehicle in a POMDP. An online solver for POMDP problems yields the optimal acceleration action for a safe manoeuvring of the vehicle through the pedestrians in real-time. However, due to computational reasons the POMDP model distinguishes only between three discrete acceleration values and follows a reference path given by a high level Hybrid A* planning algorithm.

A related approach for belief state planning in urban intersections based on discrete actions but a \textsl{continuous state and observation} space is presented by \citet{bouton_belief_2017}. The results show only minor improvements compared to a heuristic based approach using the Time To Collision (TTC). Thus, the authors propose that more realistic models could improve the performance at the expense of higher computational cost. 


\subsection{Reinforcement Learning for Autonomous Driving}

Reinforcement Learning has been applied to solve different types of motion planning tasks for autonomous vehicles.

\citet{pietquin_reinforcement_2012} use reinforcement learning to optimize the longitudinal behaviour in a driver's assistance system. The action space consists of a command for switching between two different system states and a continuous value for the acceleration, whereas the TTC of the nearest vehicle and the pedals' positions define the state space. Rewards are based on the TTC. The authors show that the learned control policy outperformed the previous standard strategy based on a priori knowledge of car and environment dynamics. Their approach is limited to problem definitions with low dimensionality, but results show that application of reinforcement learning is promising for motion planning tasks of autonomous vehicles.

\citet{li_reinforcement_2015} apply table based Q-learning for lane switching and overtaking scenarios on highways. The state space is defined by the longitudinal distance to other vehicles, relative speed and current lane number. The manually tuned reward function takes into account collisions, velocity changes, occupancy of the overtaking lane and a velocity limit. The authors constitute that the learned policy performs better than a simple expert system. However, due to computational reasons table based Q-learning allows only for a limited number of discrete actions and states, and is thus not applicable to more complex scenarios.
  
Navigating intersections using Deep Q-Learning is investigated in \cite{isele_navigating_2017}. The authors examine the performance of two different action spaces: 1) discrete acceleration and 2) wait and go commands. To define the network input, the space is discretized into a grid. Each grid cell currently occupied by a car leads to a non-zero network input consisting of the car's heading angle, velocity and TTC. Comparing the DQN approaches to a baseline method based only on the TTC for five different intersection scenarios yields better performance for the DQNs in terms of task completion. A small percentage of collisions remains for both deep neural network approaches. The authors remark that this is possibly due to discretization effects and that a longer training time may alleviate these errors. In a further study the DQN networks are trained for a specific scenario like turning left. By applying a network to a previously unseen scenario, such as turning right, the authors investigate the generalization performance. But, no network transfers well to all tasks. 

 \citet{el_sallab_deep_2017} propose a end-to-end Deep Reinforcement Learning framework for autonomous driving consisting of convolutional networks for perception and fusion tasks, recurrent networks for partially observable state estimation and Q-networks for state value estimation and action selection. In an experiment, they train a lane keeping assistant in a simulation environment.  The authors chose a simple approach for the observation model without partial observability. The network input is given by the vehicle's position between lanes and the current velocity. Thus, they do not have to apply their proposed framework and compare only Deep Q-learning and Deep Deterministic Actor-Critic approaches (see section \ref{sec:meth_rl}).

%add: \cite{shalev-shwartz_long-term_2016}

\subsection{Summary}	

State of the art path planning algorithms for autonomous vehicles require a heuristic function to guide the state exploration process and to ensure fast convergence in unstructured environments. Commonly, the heuristic estimate consists of multiple different functions each addressing a single aspect such as the non-holonomic constraints or obstacle avoidance. In general, incorporating new aspects into existing heuristic concepts, like unifying planning in both unstructured and structured environments, often requires redesign of the algorithm and careful parameterization. 
	
Probabilistic motion planning with partial observable state spaces is closely related to finding the optimal sequence of actions for a POMDP problem. In theory it can be achieved by performing value iteration over the belief distribution \cite{thrun_probabilistic_2006}. However, each value iteration step spaces requires theoretically an integration over the whole belief space.  Due to the high computational cost a feasible solution is thus only given for low-dimensional problems in case of discrete states, actions and observations. Therefore, existing probabilistic planning algorithms focus on only a subset of the different types of uncertainty being most relevant for the considered scenario and simplify the planning problem by using linearized system dynamics with Gaussian prediction models.
	
Reinforcement learning for autonomous driving mainly focuses on the field of decision making with scenarios such as lane change maneuvers or intersection crossing, where only a low number of discrete actions must be handled. Other methods target at simple planning problems such as a lane keeping assistance, where planning is not impeded by the non-holonomic constraints of the vehicle. One of the main issues is that up to now no generic approach is available making neural networks generalize well to previously unseen scenarios.

To conclude, for motion planning in autonomous driving no generic concept exists which incorporates in a versatile way the various probabilistic aspects of environmental interaction, while handling different traffic scenarios in both structured and unstructured environments. 
 
\section{Approach}
In the general reinforcement learning setting an agent receives observations from his environment, selects and performs an action and returns the next observation and a reward. Depending on the observability of the system the agent either receives the full or only partial state space knowledge and thereafter the problem can be associated with a MDP or POMDP.
 
Regarding the planned path of an autonomous vehicle as a sequence of state-action pairs allows transferring a path planning problem into a reinforcement learning problem with the goal being the estimation of an optimal policy the vehicle shall follow. As the multitude of different planning scenarios and possible vehicle states leads to a high dimensional continuous observation space, we have to apply reinforcement learning frameworks suitable for such problems. 

\subsection{Algorithms} \label{sec:meth_rl}
Value based algorithms are suitable for planning in discrete action spaces. The learned Q-function can be post-processed to yield a heuristic function or be used as a stand-alone planner. In contrast, policy search and actor-critic algorithms enable to use a continuous action space allowing the value based approach to be extended towards a versatile uncertainty planner at trajectory level. To tackle these challenges, the following algorithmic approaches may be explored within the scope of this thesis.

\subsubsection*{Value Based}

\citet{mnih_human-level_2015} introduced the biologically inspired mechanism of experience replay for Q-Learning. By that, they avoid issues with correlation of training samples when using state-action sequences of a single episode in batch learning. Further, to prevent fast error propagation, they update the target network only after a certain number of training steps. 

To avoid the issue of overestimation of the Q-Values in large scale problems \citet{van_hasselt_deep_2016} establish the concept of Double Deep Q-Networks by decomposing the optimization target into an action selection and an action evaluation function modelled by two different neural networks.

\subsubsection*{Policy Search}

Direct optimization of a parameterized policy with respect to future rewards requires less parameters compared to value based approaches and usually allows for a more straightforward integration of expert knowledge. However, model-free non-linear policy search was until recently only possible for a limited number of parameters \cite{deisenroth_survey_2013}. \citet{schulman_trust_2015} developed a bounded gradient estimation method for stochastic policies based on the Kullback-Leibler divergence to constrain the optimization procedure to only step into directions of policy improvement and successfully trained a 18-dimensional walker model based on a neural network. 

\subsubsection*{Actor-Critic}
Actor-critic approaches combine the advantages of Q-learning and policy search methods. \citet{pmlr-v32-silver14} developed an off-policy deterministic actor-critic approach and managed to train a 6-segment octopus arm with 20 action and 50 state dimensions based on a simple multilayer perceptron. \citet{lillicrap_continuous_2015} apply this approach to deep learning of continuous action policies directly from pixel inputs and scale the approach to high dimensional observation spaces. Additionally, they improve training stability based on the methods presented in \cite{mnih_human-level_2015}.    


%\rework{	
%\paragraph{stochastic vs. deterministic policy}
 %}


\subsection{Setting}

Using reinforcement learning for non-holonomic path planning problems requires an appropriate modeling of the environmontal state space, the agent's possible actions and the resulting rewards. We want to explore different settings based on kinematic or kinodynamic planning and look into discrete \cite{van_hasselt_deep_2016} or continuous action modeling \cite{mnih_asynchronous_2016}. The rewards can be adjusted based on planning results of existing planners, e.g. the Hybrid A* algorithm, or be learned via Inverse Reinforcement Learning of expert demonstrations (see section \ref{ssec:lfd}).



\subsection{Feature Representation} \label{sec:feat_rep}

The feature representation should contain enough environmental details to allow subsequent network components to integrate them into an accurate vehicle motion. Furthermore, it must include relevant information about intentions of other traffic participants at a more abstract level. High-level features such as the ego vehicle's speed could be directly used as network input and be combined with a learned feature representation which could be derived during training from the sensor inputs such as camera images or Lidar data, or from fused data in form of an occupancy map. Possible approaches for learning-based feature extraction are given in the following.
 
Frequently, convolutional architectures are applied for processing image based inputs \cite{mnih_human-level_2015,lillicrap_continuous_2015} and grid maps \cite{pfeiffer_perception_2016}. To learn a feature representation that is useful for the actual task, one can chose an architecture where the error backpropagated to the convolutional part of the network is composed of two parts \cite{lample_playing_2016}. A supervised approach guides the learning process of the feature representation to indicate, if certain objects are present in the input scene. By using additionally a reinforcement learning approach, a better feature representation for the particular task is achieved. However, feature representations based on convolutional approaches may result in a feature set which describes the environment structure only on a \textsl{local} basis. 
  
\citet{wahlstrom_pixels_2015} jointly minimize the cost function of an autoencoder and a system prediction model in a MPC algorithm. This approach enables their algorithm to learn meaningful \textsl{global} features for controlling an inverted pendulum based on image inputs.



\subsection{Network Architecture} \label{sec:net_arch}

The architecture of a deep neural network is defined by the number of fully connected and convolutional layers and their types of activation functions as well as the amount of recurrence, the branching of the network at certain points or the skipping of layers. It highly depends on the chosen reinforcement learning algorithm, feature representation and setting. The definition of a deep neural network architecture implicitly states our prior belief about the space of functions in which the learned functional representation should lie  \cite{Goodfellow-et-al-2016}. By developing a problem specific architecture we want to improve the convergence rate of training and the generalization capability of the Deep Reinforcement Learning algorithm. 

Specifically, the following architectural criteria shall be explored in detail within this thesis. Solving of POMDP problems with deep neural networks is often based on recurrent architectures to allow the network to internally build its own belief. Section \ref{sec:POMDP} describes such concepts in detail.
Apart from that, the convergence and success rate of Deep Reinforcement Learning algorithms can be improved by architectural refinements.
\citet{wang_dueling_2015} introduce a dueling architecture which uses separate branches in the network to estimate the state value and the advantage function, resulting in state of the art performance. Based on their approach, \citet{gruslys_reactor:_2017} develop a sample-efficient actor-critic network design. They define three network branches with separate estimates for the state-action value as well as for a behavioral and exploratory policy.


\subsection{Training} \label{sec:training}

The training process for reinforcement learning can be made more efficient by minimizing the amount of agent-environment interactions required for finding an optimal policy.     
We can prioritize certain experiences in the replay mechanism depending on the expected information gain of an experience as described by \citet{schaul_prioritized_2016}. Incorporating expert demonstrations into the training process allows a policy search algorithm to be guided towards regions with high rewards \cite{levine_guided_2013}. Such demonstrations could come from existing probabilistic planning algorithms or from test subjects driving in a simulator.



\subsection{Learning of the Reward Setting} \label{ssec:lfd}

The appropriate specification of the reward structure highly determines the quality of the learned policies. Therefore, methods from the field of inverse reinforcement learning could be used to learn the underlying reward structure of the reinforcement learning problems based on expert demonstrations, e.g. human driving trajectories.

\citet{abbeel_apprenticeship_2008} present an approach for learning a linearly parameterized reward model to match five different human driving styles in parking scenarios.

An arbitrary reward function of a predefined MDP can be estimated with Maximum Entropy Deep IRL by iteratively maximizing the likelihood of the expert demonstrations taking the currently learned reward setting with the associated optimal policy as a basis. \citet{wulfmeier_watch_2016} use this approach to learn cost maps for navigation of a Golf car in low-speed urban scenarios.

An application of the above methods requires enough training data, e.g. obtained from human expert demonstrations. Generating real-world driving data is time-consuming and does not allow to iteratively repeat the same scenario with fixed system and environmental properties. Thus, we may collect expert data in a driving simulator as already performed by \citet{sadigh-rss16} and \citet{vasquez_open_2014} to imitate human cooperative behavior at intersections and highway driving scenarios.

\subsection{Planning in Deep Reinforcement Learning} \label{sec:planning}

\begin{figure}
	\begingroup
	\centering 
	\scriptsize
	\def\svgwidth{8cm}
	\input{pictures/POMDP.pdf_tex}
	\endgroup
\caption{Environmental interaction in a POMDP setting: The deep neural network components of the agent may be divided into a belief state estimation part based on a recurrent architecture and a planning part for policy derivation.} \label{fig:POMDP}
\end{figure} 

There exist  Deep Reinforcement Learning approaches specifically adapted to  planning tasks which can be refined and extended.
\citet{pfeiffer_perception_2016} train a data-driven end-to-end indoor motion planner for a differential drive robot. Their supervised learning approach uses a Deep CNN to train the network in a simulation environment with a tuple of a local laser measurement, the target information and an expert steering command given by a global planner. The authors obtain convincing results also in previously unseen complex environments. However, they do not consider non-holonomic constraints.     

\citet{tamar_value_2016} develop a fully-differentiable recurrent and convolutional neural network architecture to realize a value iteration algorithm. It learns transition and reward functions with end-to-end learning.   

The predictron proposed by \citet{silver_predictron:_2016} is an architecture focusing on the estimation of state values. It is able to learn an internal state representation and a model describing state transitions and rewards. By unrolling the learned representation in a recurrent setting the predictron estimates the state value with respect to future rewards. We could extend this architecture from pure value estimation towards handling planning problems. Furthermore, the approach could be adapted to learning a mapping from the external environmental state input to an internal belief state representation.    

\subsection{Partial Observability for Deep Reinforcement Learning} \label{sec:POMDP}
 
The algorithms described in section \ref{sec:meth_rl} such as the Deep Q-Network (DQN) assume a MDP setting based on a fully observable environment. If the environmental states are only partially observable, a network input consisting of stacked past states can be used \cite{mnih_human-level_2015}. However, with such an approach a neural network is not able to effectively remember past state observations and to incorporate them into a consistent belief estimation.

To overcome these drawbacks, the Deep Reinforcement Learning community started to explore approaches for dealing with partial observability and belief state planning. 

\citet{egorov_deep_2015} demonstrates that DQNs can sucessfully learn to plan in belief space when the network input is given already in  belief state representation. In a small discrete POMDP problem they compare the learned policy to an exact solution based on the SARSOP solver. 

To integrate the history of passed observations into an internal belief representation, \citet{hausknecht_deep_2015} define a Deep Recurrent Q-Network (DRQN). Their architecture allows for better generalization performance than a DQN, when it is first trained with full observability and afterwards applied to a POMDP setting given by a partially obscured input of game screens.   
\citet{lample_playing_2016} successfully extend their approach to the more challenging task of playing a first person shooter game in a 3D environment.

\citet{zhu_improving_2017} include also the action selected at the previous timestep into the network input instead of using only the current observation  to allow the network to internally build a belief representation based on state-actions pairs. They further improve the generalization performance achieved in \cite{hausknecht_deep_2015}. 
  
In principle, the above approaches share the same architecture, depicted in figure \ref{fig:POMDP}. They use a LSTM layer for belief state estimation used by a subsequent fully connected layer for policy generation. However, the they do not explicitly address the challenge of planning within their network architecture and only rely on the LSTM layer to deal with partial observability. 

In contrast, \cite{karkus_qmdp-net:_2017} present QMDP-net, an architecture differentiating between a modelling and a planning component. It implements the QMDP algorithm, an approximate solver for POMDP problems, using a filter component which propagates the belief over time and a planner which derives the next action based on the current internal belief and environmental observation. Specifically, the planner implements value iteration in belief space similar to the approach presented in \cite{tamar_value_2016} whereas the filter component performs Bayesian filtering with convolutional operations.

It seems promising to apply, evaluate and extend the above approaches in the context of probabilistic planning for autonomous vehicles.


\subsection{Simulation Environment} \label{sec:sim_env}

We develop a simulation environment which allows to define different kinds of environmental uncertainty in two ways: 1) Specification in terms of a probability distribution, for example a Gaussian model as used for instance in obstacle tracking with Kalman filters \cite{urmson_tartan_2007} or for modeling of traffic participants \cite{brouwer_comparison_2016, lenz_deep_2017}. 2) Using an empirical distribution, describing for example the actuation uncertainty based on samples from test drives within AudiPilot. 
 
The reinforcement learning agent must internalize these uncertainty models during training. At each time step an environmental observation instance is sampled from the combined distribution and provided to the agent. We want to explore if the agent is able to infer a reasonable plan in belief space by only receiving samples of the probabilistic world model. 

The implementation may be based on one of the following existing open-source simulation platforms:
\begin{itemize}
	\item The SUMO simulator \cite{krajzewicz_recent_2012} focuses on traffic simulation in urban scenarios allowing for  specification of arbitrary road networks and signaling infrastructure based on OpenStreeMap data. It is often applied for research in the fields of decision making and cooperative planning such as in \cite{isele_navigating_2017}. However, it is based on a 2D environment and does not allow to straightforwardly specify uncertainties in sensing or acting. 
	\item Gazebo in combination with ROS is a popular framework for complex robotic simulation tasks in indoor and outdoor environments, also allowing to simulate sensor inaccuracies and noise. But so far, no useful and versatile application for research in the area of autonomous driving exists.
	\item The open source racing car simulator (TORCS) provides a python interface to control the vehicle and receive environmental information such as the current lane or the position of opponents. It is used by \citet{sallab_end--end_2016} for learning a lane keeping assistant. Drawbacks are the missing possibility to define urban scenarios or simulate environmental uncertainty.
\end{itemize} 

\section{Synergies}
This thesis would be closely linked to progress in the project AutoPilot and contribute to the establishment of a flexible simulation environment for autonomous driving at fortiss. Furthermore, fortiss as the future research center for artifical intelligence in Bavaria my benefit from building up competence in the field of Deep Reinforcement Learning. 

\subsection{AutoPilot}
Planning in narrow uncertain and unstructured environments is one of the main goals of the ongoing parking pilot project. Research for this thesis in the field of probabilistic motion planning and the parking pilot project will mutually benefit from each other to solve the following relevant work packages included in the current product specification of AutoPilot:  
\begin{itemize}
	\item Fusion of static map data and poor resolution obstacle data into a common lane graph
	\item Multi move maneuvers based on position and obstacle uncertainty
	\item Avoidance of dynamic obstacles (pedestrians, vehicles) and realization of context dependent safety margins
	\item Multi vehicle simulation environment
	\item Evaluation of Deep Learning approaches for the field of motion planning
\end{itemize} 


\subsection{ Simulation Environment at fortiss}
Within the autonomous driving group at fortiss research focuses on different aspects, such as decision making and cooperative planning, path and trajectory planning and control. To benefit mutually from new developments and research results of colleagues, the autonomous driving group at fortiss is planning to cooperatively develop a simulation environment based on ROS and Gazebo. This simulation environment will push forward the research in the field of autonomous driving at fortiss and create more visibility by making it publicly available via a open-source license and by enhancing the group's visual demonstrations of research results and developments.


\subsection{ fortiss as Bavarian Competence Center for Artificial Intelligence }

Fortiss was selected by the Bavarian Minstry of Education to establish a Bavarian competence center for artificial intelligence. Within this department fundamental principles in AI shall be carried forward aiming at successful practical cooperation with other competence fields at fortiss. In this thesis, we want to evaluate and bring forward the state of the art in Deep Reinforcement Learning algorithms in the context of motion planning for autonomous driving. The experience and results obtained here will be beneficial for the Competence Center for Artificial Intelligence .  





\section{Conclusion}
Especially in urban driving scenarios, it is crucial to consider the various probabilistic aspects of environmental interaction ranging from sensor limitations to uncertainty in intention estimation of traffic participants. 

State of the art approaches for probabilistic motion planning restrict themselves to a subset of the multitude  of possible scenarios, as a more generic approach would require to plan in a high-dimensional belief space, in which standard POMDP solvers become computationally infeasible.

However, to take the step from highly automated towards fully autonomous driving, a system must be capable of dealing with the complexity of urban scenarios. Research in this field receives great attention in these days. By exploring model-free and high-dimensional belief space planning based on Deep Reinforcement Learning for POMDP settings within this thesis, we will contribute to the relevant future developments in this area.


\printbibliography
\newpage

\begin{landscape}
	\section{Timeline}
	
	\vspace{1cm}
	
	\scalebox{0.8}{
		\begin{ganttchart}[
			vgrid={{   draw=none, dotted,  draw=none, draw=none, dotted, 
				    draw=none, draw=none, dotted, draw=none,  draw=none, black, draw=none  }},
			today=2017-10,
			today label=TODAY,
			today rule/.style={
				draw=RoyalBlue!50!black,
				dash pattern=on 3.5pt off 4.5pt,
				line width=3pt
			},
			today label font=\small\bfseries,
			progress=today,
			progress label text={},
			y unit title=0.8cm,
			y unit chart=0.8cm,
			x unit=0.33cm,
			time slot format=isodate-yearmonth,
			compress calendar,
			title/.append style={draw=none, fill=RoyalBlue!50!black},
			title label font=\sffamily\bfseries\color{white},
			title label node/.append style={below=-1.6ex},
			title left shift=.05,
			title right shift=-.05,
			title height=1,
			bar/.append style={draw=none, fill=OliveGreen!75},
			bar height=.6,
			bar label font=\color{black!70},
			group label font=\bfseries,
			group right shift=0,
			group top shift=.6,
			group height=.5,
			group peaks height=.2,
			bar incomplete/.append style={fill=Maroon}
			]{2017-02}{2022-04} % 5*12 = 60 Monate begin von Februar 2017
			\gantttitlecalendar{year} \\
			\ganttbar{Proposal}{2017-2}{2017-9} \\
			\ganttgroup{Proof of concept: heuristic learning}{2017-2}{2018-3} \\
			\ganttbar{Thesis: DQN in deterministic environments}{2017-3}{2017-10} \\
			\ganttbar{DQN as heuristic function}{2017-10}{2018-1} \\
			\ganttgroup{Interaction-aware scenarios}{2017-8}{2018-12} \\
			\ganttbar{Thesis: DQN in belief space}{2017-8}{2018-3} \\
			\ganttbar{Thesis: Multi-agent-RL for intersections }{2017-9}{2018-4} \\
			\ganttbar{Integration of belief and multi-agent planning}{2018-4}{2018-12} \\
			\ganttgroup{Benchmarking}{2018-9}{2020-5} \\
			\ganttbar{Concept}{2018-9}{2019-2} \\
			\ganttbar{Implementation and evaluation}{2019-5}{2019-11} \\
			\ganttgroup{Interaction with cognitive structure}{2019-9}{2020-10} \\
			\ganttbar{Concept}{2019-9}{2020-3} \\
			\ganttbar{Implementation and evaluation}{2020-4}{2020-10} \\
			\ganttgroup{Writing and publication}{2017-12}{2022-0} \\
			\ganttbar{Papers}{2017-12}{2018-5}  \ganttbar{}{2018-12}{2019-5} \ganttbar{}{2019-11}{2020-4} \ganttbar{}{2020-11}{2021-3}  \\
			\ganttbar{Thesis}{2020-8}{2022-0} \\
			\ganttmilestone{Submission}{2022-0}
		\end{ganttchart}
	}
\end{landscape}


==> tables/statistical_evaluation.tex <==
\begin{tabular}{lllll}
\toprule
     & sample_type &    collision_samples &    max_steps_samples &      success_samples \\
planner & results &                      &                      &                      \\
\midrule
\multirow{3}{*}{EBHS} & duration &          0.8$\pm$1.3 &          0.6$\pm$1.0 &          0.0$\pm$0.0 \\
     & num_iteration &    3350.3$\pm$5718.8 &    2129.8$\pm$4405.5 &        39.2$\pm$62.2 \\
     & path_length &         11.8$\pm$4.8 &         12.3$\pm$3.8 &         11.3$\pm$2.5 \\
\cline{1-5}
\multirow{3}{*}{HA} & duration &          0.8$\pm$1.1 &          0.9$\pm$0.6 &          0.4$\pm$0.5 \\
     & num_iteration &  23484.1$\pm$29864.7 &  23625.8$\pm$16981.4 &  10856.7$\pm$13829.3 \\
     & path_length &          9.8$\pm$3.3 &         12.3$\pm$4.4 &         11.5$\pm$2.9 \\
\cline{1-5}
\multirow{3}{*}{RL} & duration &                    - &                    - &          0.0$\pm$0.0 \\
     & num_iteration &                    - &                    - &         18.3$\pm$4.1 \\
     & path_length &                    - &                    - &         11.0$\pm$2.5 \\
\bottomrule
\end{tabular}


==> temp_methods.tex <==
\section{Method}
 
\subsection{Experience-based planning}
\subsubsection{Heuristic Search}
We formulate the heuristic search problem in a general form for arbitrary environment definitions.
We shall find an optimal path of valid environment states leading from a start state \(s_{start}\) to multiple environment goal states \(s_{goal,i}, i \in \{1,\dots,N\}\). The resulting end configuration \(s_{goal,k}\) shall be determined based on a given optimality criterion, e.g. finding the path with minimum length. 
 
In an incremental search this problem is solved in an iterative manner by building a search tree rooted at the starting state. By applying a finite set of motion primitives \(a_l, l=\{1,\dots,L\}\) from the current optimal state new child states are expanded and the tree is iteratively grown until a goal configuration is reached. In each expansion step the state with the lowest total cost 
\begin{equation}
f(s) = g(s) + h(s)
\end{equation} is selected with \(g(s)\) being the cost from the start state \(s_{start}\) to the current state \(s\) and \(h(s)\) names the cost-to-go metric or heuristic function from the current state \(s\) to the optimal goal state \(s_{goal,k}\). A closed list contains already expanded nodes. The search process is over either when the open list is empty or the number of maximum iterations is reached. 

\subsubsection{Integration of Q-function}
To ensure convergence to the optimal solution, it is crucial that the heuristic function is admissible, so is never overestimating the true cost-to-go.
For fast convergence it is important that the heuristic is close to the true value. In the limit of given the true value immediate expansion to the goal is possible. How to find a heuristic giving the true optimal value...?
 
 Outcome of this section Q(s,a) must equal h(s) -> bring in Bellman Equation/ General Reinforcement Learning

 add algorithm table
 
 
\subsubsection{Admissibility}

subsymbolic and likeli admissible heuristics
 
 \section{Experiment}
 Put concrete RL implementation to experiment section
\subsection{Algorithm}
DDQN, Learning from Demonstration

\subsubsection{Problem Definition}
Action Space,
State Space,
Rewards




